Articulate your NeRF: Unsupervised articulated object modeling via conditional view synthesis

We propose a novel unsupervised method to learn the pose and part-segmentation of articulated objects with rigid parts. Given two observations of an object in different articulation states, our method learns the geometry and appearance of object parts by using an implicit model from the first observation, distils the part segmentation and articulation from the second observation while rendering the latter observation. Additionally, to tackle the complexities in the joint optimization of part segmentation and articulation, we propose a voxel grid-based initialization strategy and a decoupled optimization procedure. Compared to the prior unsupervised work, our model obtains significantly better performance, and generalizes to objects with multiple parts while it can be efficiently from few views for the latter observation.

==> sections/03method-old.tex <==


\section{Method}

% \ks{Mutex! Making a pass through this section}


% \subsection{Problem formulation}

Let $o$ be an articulated object with $K$ rigid movable parts connected with joints allowing rotational or translational movement in 3D space. 
Assume that the object $o$ moves from an initial pose $\bm{p}$ to $\bm{p}'$ where contains the local pose for $K$ parts, each $\bm{p}_k \in \text{SE(3)}$ is a $4\times 4$ transformation matrix.
% which is parameterized with the 3D origin of the joint and 4D quaternion for rotation, or a 3D direction vector and a scalar value for translation. 
Given two sets of its images $\mathcal{I}$ and $\mathcal{I}'$ from multiple known viewpoints in respective poses $\bm{p}$ and $\bm{p}'$, our goal is to predict the relative pose $\bar{\bm{p}}$ from the motion.
Note that we assume that $K$ is known apriori.

To this end, we introduce a novel method based on analysis-by-synthesis that jointly learns to segment object parts and estimate their relative poses without their groundtruth segmentation masks or pose values, and renders them in 2D to match their images in different camera views.
As illustrated in \cref{fig:overview}, our model includes a two stage optimization.
In the first stage, we learn a `static' NeRF from a set of views including an object in a single pose to capture its 3D geometry and appearance.
The second stage starts with a part voxel initialization step to obtain an accurate initialization for the following joint pose estimation and part segmentation, which are simultaneously used in the part-aware composite rendering to reproduce the second set of views including the same object in another pose.

% Let $\mathcal{I}=\{(I_1,v_1)\dots,(I_M,v_M)\}$ and $\mathcal{I'}=\{(I'_1,v'_1)\dots,(I'_M,v'_M)\}$ be sets of image ($I$) and camera pose ($v$) pairs of an articulated object with multiple rigid parts in articulation states $\bm{a}$ and $\bm{a}'$ respectively where $M$ and $N$ denote the number of views for the respective set. Our goal is to estimate the articulation joint/motion parameters as well as novel view/articulation synthesis solely from $\mathcal{I}$ and $\mathcal{I}'$. To this end, we introduce a novel method, \jd{let's discussed the name later} based on analysis-by-synthesis that effectively models articulated objects, including objects with multiple articulated parts, in a self-supervised manner. \Cref{fig:overview} provides a schematic overview of our pipeline, which consists of three primary components: part voxel initialization, pose estimation, and part-aware composite rendering. Each of these components will be discussed in detail in the subsequent subsections.



% Our research aims to model and understand the articulation of objects solely based on image data. Specifically, we seek to comprehend and recreate the articulated states of these objects in the rendering process. We've developed a pipeline that includes part voxel initialization, motion estimation using a separate pose estimator, and segmentation-guided Neural Radiance Fields (NeRF) for the rendering of articulated objects. We designed this pipeline to efficiently understand articulation, by decoupling the part level transform estimation and part segmentation to achieve performance that's on par with current state-of-the-art image-based methods. \Cref{fig:overview} illustrates the design of our pipeline. 

% We will further explain each module in detail in the following subsections. 

 
 
 
 \begin{figure}[h]
	\centering
    \includegraphics[width=\textwidth]{figures/overview_new.pdf}
    \caption{Overview of the optimization pipeline. \ks{The text is quite small in the figure. Try to make it the same size of the main text. One tip for this is to create your figure with similar scale (in pts, ccm or inches) to textwidth and then set the fontsize (in say inkscape) to be the same as fontsize of the paper (11pt?) }}
    \label{fig:overview}
\end{figure}

% \subsection{Part-aware composite rendering}



\subsection{Part-aware NeRF}
\label{sec:part_seg}
Once the static NeRF function over $\mathcal{I}$ is learned, we freeze its parameters and append a segmentation head upon it to obtain part-level information. Then we can position movable parts to correct place during rendering by applying the inverse of part relative pose on the camera viewpoint. At last, we also correct the rendered color with a composite rendering function to integrate rays for each parts. 


\paragraph{Articulated composite rendering}
% \ks{This needs to be described better. I would suggest that we start with a high-level mathematical description of the decomposition of the NERF before explaining the transformations themselves.}
We incorporate a segmentation head $s$, instantiated as 2-layer MLP, that takes in the latent feature vector from density field of static NeRF $z(\bm{x})$ as input, and outputs a probability distribution over the number of object parts.
We denote the probability of a 3D point $\bm{x}$ to belong object part $k$ as $s[k](z(\bm{x}))$.


% Extending from the static NeRF explained above, we add a segmentation branch to enable manipulation for specific parts of the object. 
% Then, the new rendering model with segmentation branch is denoted as $f_\text{sNeRF}$ which consists of $f_\text{d}$, $f_\text{c}$ and $f_\text{seg}$. The segmentation branch takes in the feature vector $\mathbf{z}$ and outputs the part probability vector $\mathbf{s}$, denoted as $\mathbf{s} = f_\text{seg}(\mathbf{z};\theta_\text{seg})$. 

% Within the NeRF framework, we leverage segmentation masks to selectively manipulate and render specific parts of the object using a pre-trained NeRF model. This process involves generating the pixel colors of the articulated object by integrating the synthesized outputs from all individual parts.

With the part information obtained from segmentation branch, we address the difficulty of moving parts in NeRF space by applying the inverse of the estimated pose, $\bm{\hat{p}}_k^{-1}$ to the rays $r \in \mathcal{R}'$ for image set $\mathcal{I}'$, denominated as $\mathcal{\hat{R}} = \{ \bm{\hat{p}}^{-1}_k \cdot r \}_{i=1}^K$. This adjustment allows us to render the object in a new pose $\bm{p}$, which can be interpreted as change of camera viewpoints in $\mathcal{I}'$.
%we model the object pose as the inverse of changes in camera viewpoint. 
% To accommodate changes in the camera viewpoint, we apply the estimated pose transform $\bm{\hat{p}}_k$ to the original rays, denominated as $\mathcal{\hat{R}} = \{ \bm{\hat{p}}_k \circ r \}_{i=1}^K$. 
%\mathcal{\hat{R}} = \{f_\text{ray}(r, \Phi_i)\}_{i=1}^K$. 
% \ks{Why is $r$ in the set of transformed rays? This seems a little awkward}\jd{as the original ray $r$ should be responsible for rendering the static part, so we put it in the same set.} 
% Note that $\hat{bm{p}}_{K+1}$ is identity transform, which responds for the rendering of the static base part. 
% The function $f_\text{ray}$ is applied to ray $r$ to transform it for rendering of different parts. 
During rendering, the formula for transmittance is rewritten as:

%the segmentation network takes in the latent feature vector obtained from the density field network denoted as $\bm{z} = z(\bm{x})$

% selects probabilities relevant to specific rays using a designated index function $s^r = f_\text{idx}(\mathbf{s}, r)$. Then the composite transmittance in composite rendering is formulated as:

% We regard the articulation motion of the object as the inverse of camera viewpoint change. And by applying segmentation mask in the NeRF space, we can manipulate and render a specific part with the pre-trained NeRF. Thus, the pixel color of an articulated objects are obtained with by combining the results of all parts. To apply the camera viewpoint changes to the original rays, we can have a set of new rays denoted as $\mathcal{\hat{R}} = \{r, f_\text{ray}(r, \Phi_i)\}_{i=1}^{K}$, where $\Phi_i$ denotes the corresponding articulation parameter of $i^{th}$ movable part, with total $K$ movable parts. Function $f_\text{ray}$ apply the estimated transform to ray $r$ for different part rendering. The segmentation network for the NeRF is defined as $\mathbf{s} = f_\text{seg}(\mathbf{x}; \theta_\text{seg})$ with $\mathbf{s} \in \mathbb{R}^{K+1}_+$ with softmax activation. However, during the rendering, we only need to pick the probability corresponding to the ray. Thus, we define an index function as $s^r = f_\text{idx}(\mathbf{s}, r)$. 

\begin{equation}
T_i =  \sum_{j=1}^{i-1} exp(-\sum_{r \in \hat{\mathcal{R}}}(s_j^{r}[k]\sigma^{r}_j\delta^{r}_j))   
\label{eqn:transmittance_composite}
\end{equation}
where ideally, $s^{r}[k]$ functions as a binary mask to correct opacity accumulation along each ray $r \in \mathcal{\hat{R}}$ without interference from unrelated parts. 
Now the part-aware rendering function from \cref{eqn:rendering} can be rewritten as:
\begin{equation}
    \hat{C}(r) = \sum_{i=1}^{N}T_i  \sum_{r \in \mathcal{\hat{R}}}(1-exp(-s^{r}_i[k]\sigma_i^{r}\delta_i^{r}))\mathbf{c}_i^{r}
    \label{eqn:color_composite}
\end{equation}
% The segmentation network undergoes optimization through \cref{eqn:photo_metric}. 
We minimize \cref{eqn:photo_metric} to learn parameters in $s$. 

% To address occlusions of articulated parts in various states, a separate segmentation function is applied in the proposal network to derive an accurate composite PDF function, denoted by $\mathbf{\hat{s}} =f_\text{prop\_seg}(\mathbf{x};\theta_\text{prop\_seg})$. The weights in the coarse step is rewritten with \cref{eqn:transmittance_composite} and the optimization of the segmentation field within the proposal network continue as outlined in previous \cref{eqn:proposal_bound}.

To align the coarse-level sampling's density estimation with composite rendering, as detailed in \cref{eqn:color_composite}, we integrate a separate segmentation function into the proposal network. Weights for the coarse sampling step are recalculated according to \cref{eqn:transmittance_composite}. In this stage, the density field in the proposal network is fixed and we only optimize the new segmentation network by minimizing discrepancies in density distribution along a ray between the proposal network and the NeRF.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/rendering.pdf}
    \caption{Rendering pipeline: perhaps we need a better figure?}
\end{figure}

As shown above, the rendering pathway is entirely differentiable, allowing for joint optimization of segmentation branch $s$ and articulated motion parameters $\bm{\hat{p}}_k$. While joint optimization leads to simpler implementation, but we find that decoupling the pose estimation and part segmentation leads to more stable estimations. In the joint optimization process, the pose estimation relies solely on pixel-level gradients. This approach often leads to falling into local minima because it lacks sufficient local information about the object. Details on the pose estimation approach will be covered in the subsequent subsection. 

% \jd{do we need an ablation here?}
% \ks{Yes link to ablation. Also, don't make it sound all gloom and doom. Say that while this idea is simple, it is not sufficient. We identified that it works if we decouple part segmentation and pose estimation.}
% \subsection{Part voxel initialization}





\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/part_initialize.pdf}
    \caption{Part voxels initialization}
    \label{fig:part_init}
\end{figure}

\subsection{Initialization and pose estimation}
\label{sec:init_pose}
Building on the composite rendering framework for part segmentation and manipulation in NeRF, we now turn to estimating the related pose $\bm{\hat{p}}_k$. We start by generating an explicit 3D representation from the static NeRF on a uniform grid. We then render depth images from camera viewpoints in $\mathcal{I}'$, where depths corresponding to non-foreground pixels in $\mathcal{I}'$ indicate 'moved' parts. Voxels at these depths are classified as dynamic, pertaining to movable parts, while others are labeled static. Finally, we project the voxels onto the image plane to form a binary mask and optimize each part’s pose by minimizing discrepancies with the foreground mask in $\mathcal{I}'$.


\paragraph{Static Voxel Extraction} 
\label{sec:voxel_extraction}We begin by extracting a voxel representation from the static NeRF within an axis-aligned bounding box, using a grid resolution of $128^3$ to ensure uniform spacing. Grids with density values above a set threshold are marked as occupied; those below are considered empty. To refine this representation and eliminate isolated noise, we project the voxels back to the image plane using camera poses from $\mathcal{I}$, filtering out any that fall into background areas.

\paragraph{Identifying Movable Parts} With the previous extracted voxels, we now obtain a coarse classification on dynamic and static voxels. By rendering depth images from static NeRF with camera viewpoints from $\mathcal{I}'$, depth pixels falls outside the foreground areas in $\mathcal{I}'$ are identified as dynamic pixels, while others as static. Voxels associated with dynamic pixels are classified as dynamic voxels, while the rest are classified as static voxels. For objects with more then two parts, we will employ DBSCAN \cite{ester1996dbscan} to perform clustering on the dynamic voxels, and keep the largest $K-1$ clusters. 

\paragraph{Pose estimation}
\label{sec:pose_estiamtion}
We now introduce how to estimate the articulated motion parameters independent of the rendering framework. We want to project the static and dynamic voxels obtained above back to the image plane, and optimize the $\bm{\hat{p}}_k$ by matching the projection with object foreground masks in $\mathcal{I}'$. The projection for each movable part is denoted as $\mathcal{\hat{U}}_k = \bm{K}[\bm{\hat{p}}_k^{-1}\bm{v}]\mathcal{V}_k$, where $\bm{K}$ is the camera intrinsic parameter, $\bm{v}$ is the camera viwepoint, $\mathcal{V}$ is the voxels, $\mathcal{U}$ is the 2D points on the image plane. However, forming binary images with $\mathcal{U}$ is not a differentiable operation. Thus, we reframe this task as a problem of point cloud completion on the image plane. The ground truth 2D points are extracted from the foreground binary mask from $\mathcal{I}'$, denoted as $\mathcal{U}'$. Then we merge the projected 2D points from voxels as $\mathcal{\hat{U}} = \{\mathcal{\hat{U}}_k\}$. Then poses $\{\bm{\hat{p}}_k\}$ are optimized by minimizing the Chamfer distance between $\mathcal{U}'$ and $\mathcal{\hat{U}}$, formulated as: 
\begin{equation}
\{\bm{\hat{p}}_k\}^{*} = \arg\min_{\{\bm{\hat{p}}_k\}} \, f_\text{CD} (\mathcal{U}', \bar{\mathcal{U}})   
\end{equation}

% Given the camera viewpoints in the articulated image set $\mathbf{v}'$ for $M$ images, we begin by rendering images using the static NeRF model positioned at $\mathbf{p}'$. This step produces sets of 2D foreground points in both the articulated and rendered static images, denoted as $\mathcal{U}'_m$ and $\mathcal{U}_m$, respectively.

% Focusing on dynamic parts of the articulated object, we have $K$ segments with associated parameters $\Phi = \{\Phi_i\}_{i=1}^K$. A transformation derived from $f_\text{art}(v_m;\Phi_i)$, modifies the camera pose for each part resulting in updated pose $v_{m,i}$. The projection of dynamic voxels into image space is then captured by: $\mathcal{U}_{m, i}^d = f_\text{proj}(\mathcal{V}_i^d , v_{m, i})$. Combining these projections for all $K$ dynamic segments with the shared foreground locations $\hat{\mathcal{U}}_m = \mathcal{U}_m \cap \mathcal{U}_m '$ , we construct a composite set $\bar{\mathcal{U}}_m = \{ \hat{\mathcal{U}}_m, \mathcal{U}_{m, i}^d\}_{i=1}^K$. The learnable parameters $\Phi$ are optimized by minimizing the Chamfer distance between $\bar{\mathcal{U}}_m$ and $\mathcal{U}_m$, formulated as: 
% \begin{equation}
% \Phi^{*} = \arg\min_{\Phi} \, f_\text{CD} (\mathcal{U}', \bar{\mathcal{U}})   
% \end{equation}

% To tailor the model to specific types of motion, we classify the dynamic behavior into revolute and prismatic actions using an initial optimization of  $\phi$ under the $SE(3)$ group. Once the motion type is classified, we parameterize revolute motion using $\Phi_r = \{\mathbf{o}, \mathbf{q}\} \in \mathbb{R}^7$, where $\mathbf{o}$ is the origin point in the frame of the articulated part and $\mathbf{q}$ represents the quaternion for rotation. In the case of prismatic motion, the parameters $\Phi_p = \{\mathbf{u}, \alpha\} \in \mathbb{R}^4$ define movement, with $\mathbf{u}$ being the direction vector and $\alpha$ the scaling factor.

\subsection{Iterative training}

As pose estimation and part segmentation are optimized separately, a strategic approach is required to ensure convergence. We introduce a novel training methodology that alternates and iteratively optimizes both components. Initially, we follow the procedure outlined in \cref{sec:init_pose} to generate a preliminary guess for part-level voxels and part poses $\{\bm{\hat{p}}_k\}$. These estimated poses are then integrated into the composite rendering pipeline as described in \cref{sec:part_seg} for segmenting parts within the NeRF space. After several segmentation iterations, we perform a higher resolution scan of the NeRF space, similar to the steps in \cref{sec:voxel_extraction}, to predict part labels for each voxel. Voxels within a predefined distance threshold that share the same predicted label are kept to replace the previous estimated $\mathcal{V}_k$. These newly defined sets $\{\mathcal{V}_k\}$ are then used in \cref{sec:pose_estiamtion} to refine the estimates of part poses $\{\bm{\hat{p}}_k\}$, enhancing both the accuracy and detail of the segmentation and pose modeling. We repeat the pose estimation and part segmentation several times until the model converges. 

==> sections/06checklist.tex <==
\section{Checklist}

\begin{itemize}
    \item real-world object demo
    \item visualization for articulation generation
    \item ablations on whether decoupe the seg/pose estimation
    \item visualization for limitation analysis
    \item supplementary: 5-time-best joint parameter estimation results comparison with PARIS
    \item supplementary: more visualization results, compared with PARIS
\end{itemize}

==> sections/07realchecklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section*{NeurIPS Paper Checklist}

\if0
%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 
%%% END INSTRUCTIONS %%%
\fi


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Each claim is substantiated by methodological discussions in \cref{sec:method} and rigorous experiment evaluations in \cref{sec:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Details about discussions about limitations can be found in \cref{sec:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In this paper, we focus more on the practical results, which is shown in \cref{sec:exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the details about our method can be found in \cref{sec:method}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code and data will be released upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Details on the training setting is shown in \cref{sec:training_settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We ran our experiments multiple times and report average performance with the standard deviation. In addition, we report results over a set of diverse objects and evaluate them by using several metrics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report the compute resources used in our work  in \cref{sec:training_settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This project conform with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't discuss the social impact of this project in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no such risks in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We properly cited the origianl paper for the SAPIEN synthetic dataset used in our paper. The asset for SAPIEN follows the MIT license.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Codes and data will be released upon acceptance, together with instructions for use and license.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper focuses on non-living objects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper focuses on non-living objects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

